Hydration Mimicry by Membrane Ion Channels

Ions transiting biomembranes might pass readily from water through ion-specific membrane proteins if those protein channels provide environments similar to the aqueous solution hydration environment. Indeed, bulk aqueous solution is an important reference condition for the ion permeation process. Assessment of this hydration mimicry view depends on understanding the hydration structure and free energies of metal ions in water to provide a comparison for the membrane channel environment. To refine these considerations, we review local hydration structures of ions in bulk water, and the molecular quasi-chemical theory that provides hydration free energies. In that process, we note some current views of ion-binding to membrane channels and suggest new physical-chemical calculations and experiments that might further clarify the hydration mimicry view.

==> Conspectus.tex <==
%%TC:ignore
\begin{figure*}
	\includegraphics[width=0.7\linewidth]{TOC_graphics.png}
\end{figure*}
\twocolumn[ 
\section{Conspectus} 
An interesting view of ion translocation across biomembranes is that
ions readily pass from water through ion-specific  membrane proteins
when channel-lining structures provide an environment similar to the
hydration environment of ions in aqueous solution.  The local
biomolecular structure may arrange an ion binding free energy
approximately equal to the free energy of ions in bulk liquid water.
Bulk aqueous solution is thus an important reference condition for the
ion permeation process. To refine these considerations, we compare local
hydration structures of ions in bulk water, and their hydration free
energies, with ions in the binding sites of ion channels. We apply
$ab~initio$ molecular dynamics (AIMD), electronic structure
calculations, and statistical mechanical quasi-chemical theory (QCT) to
alkali metal ions (Li$^+$, Na$^+$, K$^+$, and Rb$^+$), alkaline earth
ions (\Mg, \Ca, \Sr and \Ba), and binding sites from channels selective
for \K, \Mg, or \Ca, and which can be blocked by \Ba, but not \Sr.  
Neighborship decompositions of the AIMD radial distributions are
especially helpful in defining direct solution contacts, and thus 
guiding QCT applications.
We also discuss the contribution of the electrostatic potential-of-the-phase,
spatially uniform for conducting phases, to computed single-ion free
energies. They discriminate ions at solution interfaces,
and limit the fundamental thermodynamic testing of computations.

\bigskip
Our results lead to several new conclusions. Firstly and overall, free energy
mimicry  for ion binding  to channel structures is often consistent with
ion discrimination examined here. Secondly, alternative ions of the same
size as permeable ions, but with higher charge, can be less permeable
because of stronger binding to the end-point bulk solutions. Or they can
bind more strongly to the membrane protein and block permeation.
Thirdly, hydration mimicry can occur locally, as in the case of channels
that bind the blocking \Ba~ion, and can also operate through the distant
environment, as in the case of permeant \Mg\ and \Ca\ ions that carry
along their inner-shell hydration structure.  Finally, as illustrated by
channels that provide crowded, over-coordinated binding sites for \K\
ion binding and permeation, hydration mimicry sometimes does not apply.
%\endsection*
\bigskip

\bigskip
]
%%TC:endignore

==> sec_Ion_transfer_free_energies.tex <==
a

==> sec_QCT_and_binding_sites.tex <==

\begin{figure}
\includegraphics[width=3.0in]{wat_chan_ene_V5.pdf}
\caption{Comparison of solvation free energies of  
ions in water (left) and models of K-channel binding sites (right). 
For the GG$_4$ ($\epsilon=1$) cases,  diglycine (GG) molecules model
an interior binding site of a K-channel selectivity filter.
(THR)_4, ($\epsilon=80$) cases
use four threonines to model an inner site adjacent to water, 
thus $\epsilon=80$. Except for (GG$^\ast$)$_4$, these  
models set ion-oxygen distances at about 2.8~\AA.
The (GG$^\ast$)$_4$ model locates five of the eight oxygen atoms
at about 2.4~\AA\ from the Na$^+$.  The blocking ions
(\Ba and \Sr) are not trapped, and Na$^+$ is not trapped in a
distorted binding site.}
\label{fig:wat_chan_ene_V4}
\end{figure}
 
\section{QCT AND BINDING SITES}
Here we discuss binding site models using \Ba~binding to the 
innermost binding site of K-channels (S4) as an example.  

We first construct the inner-shell solvation structure based
on information from the K-channel crystal structure with the S4 site
occupied by \Ba.  Four threonine (THR) amino acids
interact with that \Ba\ in bidentate fashion. Based on that information, we
build inner-shell clusters Ba(THR)$_{4}{}^{2+}$. To validate these models, we calculate the
root-mean-squared distance of oxygen atoms between
the THR residues of the crystal structure (PDB 1K4C) and optimized
Ba(THR)$_{4}{}^{2+}$ solution structure. All O atoms move less than 1~\AA\ after geometry
optimization.

In the QCT analysis, the density term describes the availability of
ligands to coordinate the ion.  In analogy to the hydration studies,
$\rho^{(8)}_\mathrm{TXB}$ may be taken as the density of pure liquid
threonine at standard conditions.  Liquid threonine density is the same
order of magnitude as liquid water density ($\sim$~1 g/ml).  Given that
eight (8) oxygen ligands form a stable complex around \Ba\ both in water
and in the S4 binding site, the assignment of ligand density appears
reasonable.  A precise value for $\rho^{(8)}_\mathrm{TXB}$ is
unimportant since the contribution to free energy depends only on $\ln
\rho^{(8)}_\mathrm{TXB}$.

The outer-shell terms modeled the aqueous
environment as a dielectric medium with $\epsilon=80$.  An aqueous
environment borders the S4 binding site on the intracellular side in the
form of a cavity with ~20 waters in the closed state.  In the open
state, the cavity opens to the bulk
intracellular solution.  Toward the extracellular side, a single water
borders the S4 binding site.


==> subsubsec_Theoretical_framework.tex <==
\subsubsection{Theoretical framework}
In the QCT theoretical framework used here to compute ion solvation free energies, 
constraints on the local solvation architecture, due to 
effects from the surrounding environment or intramolecular bonding within the local environment, can be taken into account naturally, along with other factors like variations in ligand chemistry and solvation properties of the environment. Those characteristics 
permit direct testing of hydration mimicry and other hypotheses about how the
structures of channels and transporters lead to rapid permeation of select ions across membranes.
Since hydration mimicry emphasizes structure, the influence of ligand chemistry
on ion binding free energies will not be addressed here, even though prior
works have studied that effect extensively.
%Bostick, australia guy, carboxylates, Sansom, Roux?

As illustrated below, the environment surrounding an ion
and its local solvation structure plays a significant role in ion solvation free energy.   The environment influences
ion solvation free energy in several ways, including through favorable
long-ranged electrostatic interactions, unfavorable effects due to
ligand desolvation from the environment prior to ligation with an ion, and potentially destabilizing
constraints applied by the environment to local solvation structure in channel binding sites. 


Before proceeding to the theoretical underpinnings of the free energy calculations used here, 
we first introduce the ions and proteins that
will be the subject of those calculations.

 %{\color {red}  citations to above are in Stevens/Rempe paper on carboxylates; 

%Besides applications in therapeutics, 
%an in-depth understanding of ion channel selectivity mechanisms for ion 
%permeation
%and blocking may facilitate the design of novel biomimetic membranes for
%specialized applications. Designing a membrane to mimic the free energy
%profiles shown in Figure~\ref{fig:Hydmim} would be a suitable strategy for
%developing those membranes. By fine-tuning the interactions between ion
%and membrane to reject particular ions from passing through, as required
%for water purification by reverse osmosis technology, or allow some ions
%to permeate, as required in water purification by electrodialysis
%technology, or separate specific ions or molecules, as needed for
%CO$_2$/CO capture,\cite{Fu:2018} better membranes may be synthesized. 

